GaitPT: Skeletons Are All You Need For Gait Recognition

The analysis of patterns of walking is an important area of research that has numerous applications in security, healthcare, sports and human-computer interaction. Lately, walking patterns have been regarded as a unique fingerprinting method for automatic person identification at a distance. In this work, we propose a novel gait recognition architecture called Gait Pyramid Transformer (GaitPT) that leverages pose estimation skeletons to capture unique walking patterns, without relying on appearance information. GaitPT adopts a hierarchical transformer architecture that effectively extracts both spatial and temporal features of movement in an anatomically consistent manner, guided by the structure of the human skeleton. Our results show that GaitPT achieves state-of-the-art performance compared to other skeleton-based gait recognition works, in both controlled and in-the-wild scenarios. GaitPT obtains 82.6% average accuracy on CASIA-B, surpassing other works by a margin of 6%. Moreover, it obtains 52.16% Rank-1 accuracy on GREW, outperforming both skeleton-based and appearance-based approaches.

==> tables/pose-estimators-ablation.tex <==
\begin{table}[hbt!]
    \begin{center}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ l | c | c | c }
         \textbf{Pose Estimation Model} & \textbf{COCO mAP} & \textbf{Gait Variation} &  \textbf{Accuracy} \\
        \hline
        \multirow{ 3}{*}{\textbf{OpenPose \cite{OpenPose:Cao}}} &  \multirow{ 3}{*}{64.2} 
          & NM & 71.71 \\
        & & BG & 59.87 \\
        & & CL & 48.84 \\
        \midrule
        
        \multirow{ 3}{*}{\textbf{AlphaPose \cite{alphapose}}} &  \multirow{ 3}{*}{72.3} 
          & NM & 75.07 \\
        & & BG & 62.77 \\
        & & CL & 56.26 \\
        \midrule
        
        \multirow{ 3}{*}{\textbf{YOLOv3 \cite{redmon2018yolov3} + HRNet \cite{sun2019deep}}} &  \multirow{ 3}{*}{77} 
          & NM & 92.01 \\
        & & BG & 79.17 \\
        & & CL & 73.52 \\
        \midrule

        \multirow{ 3}{*}{\textbf{YOLOv7\cite{wang2022yolov7} + ViTPose  \cite{xu2022vitpose}}} &  \multirow{ 3}{*}{79.8} 
          & NM & \textbf{92.97} \\
        & & BG & \textbf{81.46} \\
        & & CL & \textbf{77.42} \\
    \end{tabular}
    }
    \end{center}
    \caption{Results of the {\color{red} same baseline} trained on data obtained with different pose estimation models from CASIA-B footage. The final recognition accuracy is highly correlated (Pearson's r = 0.93) with the mAP performance of the pretrained pose estimator on the COCO benchmark \cite{lin2014microsoft}.}
    \label{tab:data_quality}
\end{table}
